Galaxy Spectra neural Network (GaSNet). II. Using Deep Learning for Spectral Classification and Redshift Predictions

Large sky spectroscopic surveys have reached the scale of photometric surveys in terms of sample sizes and data complexity. These huge datasets require efficient, accurate, and flexible automated tools for data analysis and science exploitation. We present the Galaxy Spectra Network/GaSNet-II, a supervised multi-network deep learning tool for spectra classification and redshift prediction. GaSNet-II can be trained to identify a customized number of classes and optimize the redshift predictions for classified objects in each of them. It also provides redshift errors, using a network-of-networks that reproduces a Monte Carlo test on each spectrum, by randomizing their weight initialization. As a demonstration of the capability of the deep learning pipeline, we use 260k Sloan Digital Sky Survey spectra from Data Release 16, separated into 13 classes including 140k galactic, and 120k extragalactic objects. GaSNet-II achieves 92.4% average classification accuracy over the 13 classes (larger than 90% for the majority of them), and an average redshift error of approximately 0.23% for galaxies and 2.1% for quasars. We further train/test the same pipeline to classify spectra and predict redshifts for a sample of 200k 4MOST mock spectra and 21k publicly released DESI spectra. On 4MOST mock data, we reach 93.4% accuracy in 10-class classification and an average redshift error of 0.55% for galaxies and 0.3% for active galactic nuclei. On DESI data, we reach 96% accuracy in (star/galaxy/quasar only) classification and an average redshift error of 2.8% for galaxies and 4.8% for quasars, despite the small sample size available. GaSNet-II can process ~40k spectra in less than one minute, on a normal Desktop GPU. This makes the pipeline particularly suitable for real-time analyses of Stage-IV survey observations and an ideal tool for feedback loops aimed at night-by-night survey strategy optimization.

==> author_list_2.tex <==
\author[F. Zhong et al.]{
Fucheng Zhong$^{1}$,
Nicola R. Napolitano$^{1,2}$ \thanks{E-mail: napolitano@mail.sysu.edu.cn},
Caroline Heneka$^{3}$,
Rui Li$^{4}$,
Franz Erik Bauer$^{5,6,7}$, 
Nicolas Bouche$^{8}$,
\newauthor{Johan Comparat$^{9}$},
Krogager Jens-Kristian,
Young-Lo Kim$^{10}$,
Marcella Longhetti$^{?}$,
Jonathan Loveday$^{11}$,
\newauthor{Boudewijn F. Roukema$^{12,13}$},
Benedict L. Rouse$^{5}$,
Mara Salvato$^{14}$,
Crescenzo Tortora$^{15}$,
Roberto J. Assef$^{16}$,
\newauthor{Letizia P. Cassarà},
Luca Costantin$^{17}$,
Scott Croom$^{18}$,
Luke Davies$^{?}$,
Alexander Fritz, 
Guillaume Guiglion$^{19,20,21}$,
\newauthor{Andrew Humphrey$^{22,23,24}$},
Emanuela Pompei$^?$, 
Claudio Ricci$^{25}$,
Cristóbal Sifón$^{26}$,
Elmo Tempel$^{27}$,
Tayyaba Zafar$^{28}$
\\
% List of institutions
$^{1}$ School of Physics and Astronomy, Sun Yat-sen University, Zhuhai Campus, 2 Daxue Road, Xiangzhou District, Zhuhai, P. R. China \\
$^{2}$Department of Physics E. Pancini, University Federico II, Via Cinthia 6, 80126-I, Naples, Italy\\
$^{3}$Institute of Theoretical Physics, University of Heidelberg, Philosophenweg 12, room 306b, 69120 Heidelberg \\
$^{4}$National Astronomical Observatories, Chinese Academy of Sciences, 20A Datun Road, Chaoyang District, Beijing, China \\
$^{5}$ Instituto de Astrof{\'{\i}}sica and Centro de Astroingenier{\'{\i}}a, Facultad de F{\'{i}}sica, Pontificia Universidad Cat{\'{o}}lica de Chile, Campus San Joaquín, \\ Av. Vicuña Mackenna 4860, Macul Santiago, Chile, 7820436 \\
$^{6}$ Millennium Institute of Astrophysics, Nuncio Monse{\~{n}}or S{\'{o}}tero Sanz 100, Of 104, Providencia, Santiago, Chile \\ 
$^{7}$ Space Science Institute, 4750 Walnut Street, Suite 205, Boulder, Colorado 80301 \\
$^{8}$ Centre National de la Recherche Scientifique (CNRS), Centre of Research in Astrophysics of Lyon (CRAL), 9 av Charles André, F-69230 Saint Genis Laval \\
$^{9}$ Max-Planck-Institut für Extraterrestrische Physik (MPE), Giessenbachstrasse 1, 85748 Garching bei München, Germany \\ 
$^{10}$ Department of Physics, Lancaster University, Lancs LA1 4YB, UK \\
$^{11}$ Astronomy Centre, University of Sussex, Falmer, Brighton, BN1 9QH, UK \\
$^{12}$ Institute of Astronomy, Faculty of Physics,
        Astronomy and Informatics, Nicolaus Copernicus
        University, Grudziadzka 5, 87-100 Toru\'n, Poland \\
$^{13}$ Univ Lyon, Ens de Lyon, Univ Lyon1, CNRS, Centre de
            Recherche Astrophysique de Lyon UMR5574, F--69007, Lyon,
            France \\
$^{14}$ Max-Planck-Institut für extraterrestrische Physik (MPE), Gießenbachstraße 1, D-85748 Garching bei München, Germany \\
$^{15}$ INAF - Osservatorio Astronomico di Capodimonte, Salita Moiariello 16, 80131, Napoli (Italy) \\
$^{16}$ Instituto de Estudios Astrofísicos, Facultad de Ingeniería y Ciencias, Universidad Diego Portales, Av. Ejército 441, Santiago, Chile \\
$^{17}$ Centro de Astrobiología, Instituto Nacional de Técnica Aeroespacial, Madrid, Spain \\
$^{19}$ Zentrum f\"ur Astronomie der Universit\"at Heidelberg, Landessternwarte, K\"onigstuhl 12, 69117 Heidelberg, Germany \\
$^{20}$ Max Planck Institute for Astronomy, K\"onigstuhl 17, 69117, Heidelberg, Germany \\
$^{21}$ Leibniz-Institut f{\"u}r Astrophysik Potsdam (AIP), An der Sternwarte 16, 14482 Potsdam, Germany \\
$^{22}$ Instituto de Astrof\'{i}sica e Ci\^encias do Espa\c{c}o, Universidade do Porto, CAUP, Rua das Estrelas, Porto, 4150-762, Portugal \\
$^{23}$DTx -- Digital Transformation CoLab, Building 1, Azur\'em Campus, University of Minho, 4800-058 Guimar\~aes, Portugal \\
$^{24}$Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Universidade do Porto, CAUP, Rua das Estrelas, PT4150-762 Porto, Portugal \\
$^{25}$ Instituto de Estudios Astrofísicos, Facultad de Ingeniería y Ciencias, Universidad Diego Portales (UDP), Santiago de Chile \\
$^{26}$ Instituto de Física, Pontificia Universidad Católica de Valparaíso \\
$^{27}$Tartu Observatory, University of Tartu, Observatooriumi 1, 61602 Tõravere, Estonia
Estonian Academy of Sciences, Kohtu 6, 10130 Tallinn, Estonia \\
$^{28}$ Faculty of Science and Engineering, School of Mathematical and Physical Sciences, Level 5, Room 505, 12 Wally's Walk, Macquarie University, NSW 2109, Australia
}
